MorphoStyle: Motion Style Transfer with Morphology Control

Human motion may be viewed as a combination of action content, style, and body morphology. Existing motion style transfer methods transfer a reference style onto a content motion while assuming a canonical body, whereas shape-aware motion generators adapt motion to a target shape without explicit style control. This separation of motion style and shape (morphology) makes it difficult to generate stylized motions for non-canonical bodies; naively combining a style transfer module with a shape-aware generator often leaks action content from the style reference and disrupts shape-consistent kinematics. We present MorphoStyle, a framework for shape-aware motion style transfer that is built on a shape-conditioned Finite-Scalar-Quantization Variational Auto-Encoder (FSQ-VAE). The key contribution is to pose the desired style transfer as modular latent disentanglement comprising: (i) a contrastive style encoder that extracts content-decoupled style embeddings; (ii) a text-guided style-routing mechanism that locates style-relevant joints in a text-motion feature space; and (iii) a manifold preserving style modulator that injects discriminative style embeddings in content features as a temporally-gated low-rank offset. Extensive experiments on benchmark datasets demonstrate that MorphoStyle outperforms competing baselines in terms of both shape control and motion style transfer, while simultaneously providing quantitative shape control. For more details, please see project website: https://github.com/funkdub/MorphoStyle.

==> tables/table3.tex <==
\begin{table}[hbpt]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Training set} & \textbf{SRA$\uparrow$}
                      & \textbf{FID$\downarrow$}
                      & \textbf{Foot Skate$\downarrow$} \\
\midrule
100Style only                  & 90.3\%          & 29.80          & 0.145          \\
100Style~+~HumanML3D           & 70.5\%          & 4.01           & 0.104          \\
100Style~+~HumanML3D~+~Cross   & 68.3\%          & \textbf{3.46}  & \textbf{0.085} \\
\bottomrule
\end{tabular}
\caption{Training-data ablation. Adding HumanML3D as an unstylized diversity prior, together with cross-domain content/style sampling, trades a small amount of style accuracy for a large improvement in realism and physical plausibility.}
\label{tab:data}
\end{table}

==> tables/table4.tex <==
\begin{table}[hbpt]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Injection} & \textbf{SRA$\uparrow$} & \textbf{FID$\downarrow$}
                   & \textbf{Foot Skate$\downarrow$} \\
\midrule
Addition             & 44.7\%          & 9.13          & 0.167          \\
Low-rank Add         & 44.8\%          & 8.77          & 0.165          \\
AdaIN                & 63.8\%          & 7.21          & 0.101          \\
\textbf{FiLM} (ours) & 68.3\%          & \textbf{3.46} & \textbf{0.085} \\
Cross-Attention      & \textbf{72.2\%} & 5.10          & 0.108          \\
\bottomrule
\end{tabular}
\caption{Style injection mechanism. FiLM offers the best overall balance between style fidelity, realism and foot-skating; Cross-Attention is reported as an upper bound on style accuracy at the cost of realism.}
\label{tab:inj}
\end{table}
